Hashing for Sampling-Based Estimation

Hash-based sampling and estimation are common themes in computing. Using hashing for sampling gives us the coordination needed to compare samples from different sets. Hashing is also used when we want to count distinct elements. The quality of the estimator for, say, the Jaccard similarity between two sets, depends on the concentration of the number of sampled elements from their intersection. Often we want to compare one query set against many stored sets to find one of the most similar sets, so we need strong concentration and low error-probability. In this paper, we provide strong explicit concentration bounds for Tornado Tabulation hashing [Bercea, Beretta, Klausen, Houen, and Thorup, FOCS'23] which is a realistic constant time hashing scheme. Previous concentration bounds for fast hashing were off by orders of magnitude, in the sample size needed to guarantee the same concentration. The true power of our result appears when applied in the local uniformity framework by [Dahlgaard, Knudsen, Rotenberg, and Thorup, STOC'15].

==> Notes/Ioana_and_Jakob_s_Writeup.tex <==
\newpage
\section{Lower Tail Chernoff}


\medskip
Let $\barh:\Sigma^c \rightarrow \Sigma \times \calR$, $T_{d}:\Sigma \rightarrow \calR$ be such that $h(x) = \barh(x)_{(2)} \xor T_d(\barh(x)_{(1)})$. Then we define $$X_\alpha = \set{x\in \Sigma^c \mid \barh(x)_{(1)} = \alpha \text{ and $x$ is selected} } \;.$$
\medskip\noindent 
Let $G_{\lambda} =(e^{ \lambda \mu/\ssigma}  - \lambda \mu/\ssigma -1 )/ ( \mu/\ssigma)^2 $ and note that, since $\mu/\ssigma \leq 1/2$, we have that
$$G_\lambda \leq 4(e^{\lambda/2}-\lambda/2-1)\;.$$

\subsection{First part}
\begin{lemma}
$$\Prpc{\barh\times T_d}{ \max_{\alpha} X^2_{\alpha} \geq \tau_1}$$
\end{lemma}
\begin{proof}
\begin{align*}
\Prpc{\barh\times T_d}{ \max_{\alpha} X^2_{\alpha} \geq \tau_1} &\leq \size{\Sigma} \cdot \Prpc{\barh\times T_d}{ X_{\alpha} \geq \sqrt{\tau_1}}\\
&\leq 
\end{align*}
\end{proof}

\begin{lemma}
$$ \Prpc{\barh\times T_d}{\sum_{\alpha} X^2_{\alpha} \geq  \tau_2 }$$
\end{lemma}
\subsection{Second part}
\begin{lemma}
%\begin{align*}
%	\Prp{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu \wedge \calA}&\leq \Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \exp\Big( -\lambda^2\cdot G_{\lambda} \cdot \Big(  \sum_{\alpha}\EEpconddt{X_\alpha^2}{\barh}- \mu^2/\ssigma \Big)   -\lambda \mu \eps \Big)\Bigg] } 
%\end{align*}
\begin{align*}
	\Prp{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu \wedge \calA}&\leq \Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \exp\Big( \lambda^2 \cdot G_{\lambda} \cdot \Big(  \sum_{\alpha}\EEpconddt{X_\alpha^2}{\barh}- \mu^2/\ssigma \Big)   -\lambda \mu \eps \Big)\Bigg] } 
\end{align*}
\end{lemma}
\begin{comment}
\begin{proof}
Let \(\Xab = X_{\alpha} - \mu/\ssigma\).
    \begin{align*}
        \Prp{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu \wedge \calA}
        &= \Epph{\Prpconddt{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu \wedge \calA}{\barh}} & \text{Law of total expectation} \\
        &= \Epph{\indicator{\calA}\Prpconddt{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu}{\barh}} & \indicator{\calA} \text{ is constant when \(\barh\) is fixed} \\
    	&= \Epph{[\calA]\Prpconddt{\sum_\alpha (X_{\alpha} - \mu/\ssigma) \leq -\eps\mu}{\barh}}\\
        &= \Epph{[\calA]\Prpconddt{e^{-\lambda \sum_\alpha \Xab} \geq e^{\lambda\eps\mu}}{\barh}} &\text{for any $\lambda > 0$}\\
        &\leq \Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \EEpconddt{e^{ -\lambda \sum_{\alpha} \Xab        }} {\barh}     \cdot e^{-\lambda \mu \eps} \Bigg] } &{\text{Markov and $\calA$}}\\
        &=  \Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \prod_{\alpha} \EEpconddt{e^{ -\lambda \Xab        }} {\barh}     \cdot e^{-\lambda \mu \eps} \Bigg] } &{\text{indep $X_{\alpha}$}}
    \end{align*}


\begin{align*}
	e^{ -\lambda\Xab} &= 1-\lambda \Xab + \lambda^2 \cdot \Xab^2\cdot \frac{e^{ -\lambda \Xab}  + \lambda \Xab -1 }{\lambda^2 \cdot \Xab^2}\\
	&\leq 1-\lambda \Xab  + \lambda^2 \cdot \Xab^2\cdot \frac{e^{ \lambda \mu/\ssigma}  - \lambda \mu/\ssigma -1 }{\lambda^2 \cdot ( \mu/\ssigma)^2} & X_\alpha \geq 0 \text{ so } \Xab \geq - \mu/\ssigma\\
	& = 1-\lambda \Xab + \lambda^2\cdot  G_{\lambda} \cdot \Xab^2
 \end{align*}
 \begin{align*}
 \Epconddt{e^{ -\lambda\Xab}}{\barh} &\leq 1- \lambda \Epconddt{\Xab}{\barh} + \lambda^2\cdot G_{\lambda} \cdot \Epconddt{\Xab^2}{\barh} \\
	&\leq \exp\left(-\lambda \Epconddt{\Xab}{\barh} + \lambda^2\cdot  G_{\lambda} \cdot \Epconddt{\Xab^2}{\barh} \right) & {1+K \leq \exp(K)}
\end{align*}



\begin{align*}
	\prod_{\alpha}\Epconddt{e^{ -\lambda \Xab} }{\barh} 
	&\leq \prod_{\alpha} \exp\Big( -\lambda \cdot \EEpconddt{\Xab}{\barh} +\lambda^2\cdot  G_{\lambda} \cdot \EEpconddt{\Xab^2}{\barh}\Big) \\
	&= \exp\Big( -\lambda \cdot \sum_{\alpha}\EEpconddt{\Xab}{\barh} +\lambda^2\cdot  G_{\lambda} \cdot \sum_{\alpha}\EEpconddt{\Xab^2}{\barh}\Big) \\
	&= \exp\Big( \lambda^2\cdot  G_{\lambda} \cdot \sum_{\alpha}\EEpconddt{\Xab^2}{\barh}\Big) & \sum_{\alpha}\EEpconddt{\Xab}{\barh} = 0 \\
	&=  \exp\Big( \lambda^2\cdot  G_{\lambda} \cdot \sum_{\alpha}\EEpconddt{(X_\alpha - \mu/\ssigma)^2}{\barh}\Big) \\
	&= \exp\Big( \lambda^2\cdot G_{\lambda} \cdot \Big(  \sum_{\alpha}\EEpconddt{X_\alpha^2}{\barh}- \mu^2/\ssigma \Big)\Big)
\end{align*}

\begin{align*}
	\Prp{\sum_\alpha X_{\alpha} \leq (1-\eps)\mu \wedge \calA}&	\leq \Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \prod_{\alpha} \EEpconddt{e^{ -\lambda \Xab        }} {\barh}     \cdot e^{-\lambda \mu \eps} \Bigg] } \\
	&\leq 	\Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \exp\Big( \lambda^2\cdot G_{\lambda} \cdot \Big(  \sum_{\alpha}\EEpconddt{X_\alpha^2}{\barh}- \mu^2/\ssigma \Big)\Big)   \cdot e^{-\lambda \mu \eps} \Bigg] } \\
	&=	\Epph{[\calA]\Bigg[\inf_{\lambda\geq 0}   \exp\Big( \lambda^2\cdot G_{\lambda} \cdot \Big(  \sum_{\alpha}\EEpconddt{X_\alpha^2}{\barh}- \mu^2/\ssigma \Big)   -\lambda \mu \eps \Big)\Bigg] }
\end{align*}
\end{proof}
\end{comment}

\medskip\noindent
We let $Y(\barh) = \sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} - \sqrt{2\cdot \sum_{\alpha} \Varconddt{X_{\alpha}^2}{\barh}}$.

\begin{lemma}\label{lemma:linkexperiment}
	\begin{align*}
		 \Prph{Y(\barh) \geq \tau} &\leq 2\cdot 	\Prpc{\barh\times T_d} {\sum_{\alpha} X^2_{\alpha} \geq \tau}
	\end{align*}
\end{lemma}
\begin{comment}
\begin{proof}

	\begin{align*}
			\Prpc{\barh\times T_d} {\sum_{\alpha} X^2_{\alpha} \geq \tau} &\geq \Prpc{\barh\times T_d} {\sum_{\alpha} X^2_{\alpha} \geq Y(\barh) \wedge Y(\barh) \geq \tau}\\
			&= \Epph{\Prpconddt{\sum_{\alpha} X^2_{\alpha} \geq Y(\barh) }{\barh} \big[ Y(\barh) \geq \tau \big] } & \text{Law of total expectation}
	\end{align*}
Chebyshev's:
\begin{align*} 
	\Prpconddt{\sum_{\alpha} X^2_{\alpha} \geq Y(\barh) }{\barh}&= \Prpc{T_d}{\sum_{\alpha} X^2_{\alpha} \geq  \sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} - \sqrt{2\cdot \sum_{\alpha} \Varconddt{X_{\alpha}^2}{\barh}}} \geq 1/2
\end{align*}
% Note that this is not a claim on \(\barh\). Rather, \(\Prpconddt{\sum_{\alpha} X^2_{\alpha} \geq Y(\barh)}{\barh} \geq 1/2\) regardless of the value of \(\barh\).
Therefore:
\begin{align*}
	\Prpc{\barh\times T_d} {\sum_{\alpha} X^2_{\alpha} \geq \tau} &\geq 1/2 \cdot \Epph{ Y(\barh) \geq \tau}  = 1/2 \cdot \Prpc{\barh}{ Y(\barh) \geq \tau}
\end{align*}

\end{proof}
\end{comment}

\begin{lemma}
	\begin{align*}
		\Prph{\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \geq \tau}&\leq 
	\end{align*}

\begin{proof}

\medskip
Notice the following:
\begin{align*}
\Prph{\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \geq \tau_3 } &\leq \Prpc{\barh\times T_d}{ \max_{\alpha} X^2_{\alpha} \geq \tau_1} + \Prph{\sum_{\alpha}  \Epconddt{X_{\alpha}^2}{\barh} \geq \tau_3 \wedge (\max_{\alpha} X^2_{\alpha} \leq \tau_1)}
\end{align*}

\medskip
Then we have that:
	\begin{align*}
		\Varconddt{X_{\alpha}^2}{\barh} &\leq \tau_1 \cdot \Epconddt{X_{\alpha}^2}{\barh}
	\end{align*}
We therefore get that, for any $\tau_2$
\begin{align*}
	\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} &\leq \tau_2  + \sqrt{2\cdot \sum_{\alpha} \Varconddt{X_{\alpha}^2}{\barh}} \implies
	\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} &\leq 	 \tau_2  +\sqrt{2\tau_1 \sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh}}
\end{align*}
and futhermore,
\begin{align*}
	\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} &\leq 	 \tau_2  +\sqrt{2\tau_1 \sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh}} \implies 	\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \leq \tau_3\;,
\end{align*}

\noindent
where  $\tau_3 = 1/4  \cdot (\sqrt{2\tau_1 + \tau_2} + \sqrt{2\tau_1})^2$.
\jonas{I need to double-check this one. I get \(4\tau_2\) in the expression.}
Conversely, we have that

\begin{align*}
\Prph{\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \geq \tau_3 \wedge (\max_{\alpha} X^2_{\alpha} \leq \tau_1)}
&\leq \Prph{	\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \geq 	 \tau_2  +\sqrt{2 \sum_{\alpha}\Varconddt{X_{\alpha}^2}{\barh}} }\\
	&\leq  2\cdot \Prpc{\barh \times T_d}{\sum_{\alpha} X^2_{\alpha} \geq  \tau_2 } \qquad\qquad  \text{(\Cref{lemma:linkexperiment})}
\end{align*}

\medskip\noindent

Notice the following:
\begin{align*}
\Prph{\sum_{\alpha} \Epconddt{X_{\alpha}^2}{\barh} \geq \tau_3 } &\leq \Prpc{\barh\times T_d}{ \max_{\alpha} X^2_{\alpha} \geq \tau_1} + \Prph{\sum_{\alpha}  \Epconddt{X_{\alpha}^2}{\barh} \geq \tau_3 \wedge (\max_{\alpha} X^2_{\alpha} \leq \tau_1)}\\
&\leq \Prpc{\barh\times T_d}{ \max_{\alpha} X^2_{\alpha} \geq \tau_1} +  2\cdot \Prpc{\barh\times T_d}{\sum_{\alpha} X^2_{\alpha} \geq  \tau_2 }
\end{align*}
\end{proof}
\end{lemma}







==> Notes/Mikkel_s_Writeup.tex <==
\newpage
\subsection{Mikkel's Lower Tail Chernoff}
\paragraph{The last characters in parallel}
A simple note is that if we want the lower tail bound, then we can right as well have the last three characters in parallel, since we do not use the last character
for the independence in the first experiement

\paragraph{New ideas... they will only locally change/improve things, not change the essential parts.} we are probably much better off analyzing using Bernstein's inequality, e.g., from Wiki, 
let $X_1, \ldots, X_n$ be independent zero-mean random variables. Suppose that 
$\displaystyle |X_{i}|\leq M$ for all
$i$. Let $X=\sum_i X$. Then, for all positive 
$t$,
\[\Pr[X\geq t]\leq \exp\left(-\frac{t^2/2}{\sum_i \E[X_i^2]+Mt/3}\right).\]
With non-zero means, we essentially just
replace $\E[X_i^2]$ with $\Var[X_i]$, and with independence, $\sum_i \Var[X_i]=\Var[X]$. For
lower-tail, we use this 
to look at the probability that
\[\Pr[X\leq\E[X]-t]\]
In our case, the index $i$ is a character
$a\in \Sigma$ and $X_a$ the number of keys selected with last character $a$. 

Now some rough estimates. We are considering only the case where $\size\Sigma/4\leq \E[X]\leq \size\Sigma/2$ (since we can randomly subselect on more bits later).
Marginally, each $X_a$ is Poisson distributed with mean and variance
$\mu/\Sigma$. Thus we would like to
argue that $\Var[X]\lesssim \mu$ and
\[\sum_a \E[X_a^2]\lesssim \mu (1+\mu/\Sigma).\]


In experiment 2, we have perfect independence between the $X_a$ but we use 
experiment 1 to bound $\sum_a \E[X_a^2]$ for experiment 2.

In experiment 1, we know that with high
probability the total number of selected
keys is $\tilde\mu=(1+o(1))\mu$. When first they
have been selected, we know they 
distribute completely randomly between
the keys. This gives a Poisson distribution on each $X_a$, and the $X_a$ are negatively correlated, so this should
give us a good high probability bound
\[\sum_a X_a^2\lesssim \mu (1+\mu/\Sigma)\]
The relation to experiment 1 should then
give that for experiment 1 with its independent variables, we expect\[\sum_a \E[X_a^2]\lesssim \mu (1+\mu/\Sigma)\]
and hence 
\[\sum_a \Var[X_a]\lesssim \mu.\]
Together with the Berstein inequality above,
we should be able to prove something in the style of ,
\[\Pr[X<(1-\delta)\mu]\leq \exp(-\mu\delta^2/3)+A(3/\Sigma)^{d-3}.\]
Above, with normal Chernoff lower tail
we have $\exp(-\mu/\delta^2/2)$ and substituting $1/2$ with $1/3$ should give us sufficient wiggle room.


Now, for all the relations, one primitive
strategy is for each integer value $x\leq \log \size\Sigma$, to prove that 
\[\sum_{a\in\Sigma} [X_a=x].\]
behaves well between the two experiments. I can see how to do that, and this would suffice, but there may be a more direct approach not splitting into values $x$.
On the other hand, working with each value separately is quite easy, since we just need to count the number of buckets with
this number of selected keys. Even
though they are not independent if we consider one bucket at the time, we get concentrations via Azuma's martingale inequality... Again, the point is to show good concentration on the second moment around the true random value.

\paragraph{Further thoughts}
Actually, it is much easier to work with
the sums $\sum_{a\in \Sigma}[X_a\geq k]$.
Note that when the $X_a$ are independent
as in the last part of Experiment 2,
then the value we would like to bound is
\[\sum_a \E[X_a^2]=\sum_{k=1}^\infty
\E[\sum_a [X_a\geq k](k^2-(k-1)^2)=\sum_{k=1}^\infty
(2k-1)\E[\sum_a [X_a\geq k].
\]
We claim that w.h.p. over the first part
of experiment 2,
\[\E[\sum_a [X_a\geq k]\lesssim
\size\Sigma P(f,k).\]
where $P(f,k)$ is the accumulated Poisson distribution 
\[P(f,k)=\sum_{j\geq k}\frac{f^j e^{-f}}{j!}\textnormal,\]
with mean $f=\mu/\size\Sigma$.
If we can show that 
\[\E[\sum_a [X_a\geq k]\leq
\size\Sigma P(f,k)+\Delta_k.\]
Then we get that 
\[\sum_a \E[X_a^2]\leq \mu (1+\mu/\Sigma)+\sum_{k=1}^{\infty}(2k-1)\Delta_k.\]
Here the $\Delta_k$ will end up small and we do not need to consider larger $k$.

To prove this, we first give high probability bounds for 
$\sum_a [X_a\geq k]$ in experiment
1. We know that this corresponds to
placing a bit more than $\mu$ balls
between the bins. The probability
that a given bin $a$ gets $[X_a\geq k]$
is $P(f,k)$, and the $[X_a\geq k]$ are negatively correlated, so w.h.p., we 
end up with 
\[\sum_a [X_a\geq k]\leq
\size\Sigma P(f,k)+\sqrt{\size\Sigma P(f,k) \log\Sigma}.\]
As discussed earlier, the high probability
bound for Experiment 1 translates into a high probability bound for the expectation
in the last part of Experiment 2, so
we end up with $\Delta_k=O(\sqrt{\size\Sigma P(f,k) \log\Sigma})$. This should end up very nicely even for fairly small $\size\Sigma$, perhaps even for
$\size\Sigma=2^8$.

Also, we should do the accounting the the whole way up to what is the largest bucket size $k$. For any $k$, getting $k$ in
some bucket happens wit probability $(ef/k)^k$, so $k\sim d\log\size\Sigma/\log\log\size\Sigma$
would do. In fact, buckets of
size larger than $\log\log\size\Sigma$ will have very little influence since there are so few of them.

\paragraph{Tried to formalize the connection between Experiment 1 and 2}
The experiments involve the same random variables, but the ordering of fixing
the random variables lead to different types of bounds that we have to connect.

Define
\[X_{\geq k}=\sum_{a\in\Sigma}[X_a\geq k].\]
Analyzing Experiment 1, we showed that for some concrete value $\mu^+_{\geq k}$
and a concrete small probability bond $P_{\geq k}$,
\[\Pr[X_{\geq k}>\mu^+_{\geq k}]\leq P_{\geq k}.\]

In Experiment 2, after first part, define
\[Y_{\geq k}=\E[X_{\geq k}].\]
Now $Y_{\geq k}$ fixed for the last part of Experiment 2. In
this last part, $X_{\geq k}$ is settled as
a sum of independent 0-1 variables. By Chernoff, with $\delta=\sqrt{1/Y_{\geq k}}$,
\[\Pr[X_{\geq k}\leq (1-\delta)Y_{\geq k}]\leq \exp(-\delta^2Y/2)=1/\sqrt{e}.\]
Thus,
\[\Pr[X_{\geq k}> Y_{\geq k}-\sqrt{Y_{\geq k}}]\geq 1-1/\sqrt{e}\]
The important thing is that this holds regardless of the value of $Y_{\geq k}$.

To connect to the $P_{\geq k}$ from Experiment 1,
we note that
\begin{align*}
  \Pr[X_{\geq k}> \mu^+_{\geq k}]&\geq\Pr[X_{\geq k}>(Y_{\geq k}-\sqrt{Y_{\geq k}})>\mu^+_
{\geq k}]\\
  &=\Pr[Y_{\geq k}-\sqrt{Y_{\geq k}}>\mu^+_{\geq k}]\cdot \Pr[Y_{\geq k}-\sqrt{Y_{\geq k}}
<X_{\geq k}\mid Y_{\geq k}-\sqrt{Y_{\geq k}}>\mu^+_{\geq k}]\\
  &\geq \Pr[Y_{\geq k}-\sqrt{Y_{\geq k}}>\mu^+_{\geq k}]\cdot (1-1/\sqrt e)
\end{align*}
Thus we conclude that
\[\Pr[Y_{\geq k}-\sqrt{Y_{\geq k}}>\mu^+_{\geq k}]\leq P_{\geq k}/(1-1/\sqrt e)\]


\drop{
\paragraph{Better probability bounds}
I am thinking of ways to get better
bounds. For now just internal Mikkel note. This is something we can do as
a refinement on the end. For now,
I am just thinking of bounds
$\Pr[X_{\geq k}\geq\mu^+_{\geq k}]$.
Currently we first bound $\Pr[X\geq\mu^+]$, next 
$\Pr[X_{\geq k}\geq\mu^+_{\geq k}\mid X\leq\mu^+]$.
However, we can also look at the probability that the sum of errors (keep $k$ fixed) is bounded. The dominant
case would essentially be  $X$ and $X_{\geq k}$ deviated by the same number of standard deviations, and then
we would look at the product
$\Pr[X\geq\mu^+]\cdot\Pr[X_{\geq k}\geq\mu^+_{\geq k}\mid X\leq\mu^+]$.
If we have some targer error probability
$P$, we should exploit that error
event is the product of sub error events.
For given values of $\mu$}

\paragraph{An internal Mikkel note that I will explain later}
Currently we first bound $\Pr[X\geq\mu^+]$, next 
$\Pr[X_{\geq k}\geq\mu^+_{\geq k}\mid X\leq\mu^+]$.
In bother cases we are looking at getting
some number of standard deviations $t_1$ and $t_2$ respectively. However, what really matters to us is the sum, and to get $t_1+t_2\geq t$,
we need $\floor{t_1}+\floor{t_2}\geq \floor{t-1}$.
Thus, it suffices to consider all
integers $i+j=\floor{t-1}$ and ask
for $t_1\geq i$ and $t_2\geq j$. Now
we get to multiply the error probabilities,
essentially saving a factor 2 in the number of standard deviations for our bounds on $Y_{\geq k}$, and we can further include the last part of exerpiment 2, so we end up saving almost a factor 3 in each part. This is something I will explain further, and that we can do later in an almost black-box fashion without changing anything else.

Explain motivation a bit more.
Suppose we get $X\geq (1+\delta_1)\mu$. Suppose further that we get variance $\sigma^2$ from first part of experiment 2 (using the our subtle connection to experiment 1) bigger by an additional factor $(1+\delta_2)$, that is,
it becomes $(1+\delta_1)(1+\delta_2)\mu$. Finally
in the last part of experiment 2, using Bernstein, suppose we $X<\mu-\delta_3\sigma^2=
(1-\delta)\mu$ where
$\delta=\delta_3(1+\delta_1)(1+\delta_2)$. All of
these $\delta_i$ lead to
an error probability factor of around $\exp(-\mu\delta_i^2)$, but $\delta_3$ has much bigger
impact on $\delta$, so for a given $\delta$, we get by far the largest error probability with $\delta_1\approx \delta_2\approx 0$ and $\delta_3\approx \delta$. This means that our overall bound gets very close to that with full randomness.

Let me try to to explain in more detail with a slightly 
simplified/fake situation. Let
$Y$ be the the variance after
first part of experiment 2.
Suppose
\[\Pr[Y\geq(1+\delta_1)
\mu]= F_1(\delta_1)=\exp(-\mu\delta_1^2).\]
Also, for given $Y$, suppose
\[\Pr[X\leq \E[X]-\delta_2 Y]= F_2(\delta_2)=\exp(-\mu\delta_2^2).\]
The above inequalities correspond to
$X\leq \E[X]-\delta\mu$
where 
\[\delta=(1+\delta_1)\delta_2\iff
\delta_2=\delta/(\delta_1
+1).\]
For simplicity, we just used
$F_1=F_2$ and note we have
frequency
\[f_i(\delta_i)=-F_i'(\delta_i)=2\mu\delta_i\exp(-\mu\delta_i^2).\]
Now 
\begin{align*}\Pr[X\leq \E[X]-\delta \mu]&=F(\delta)\\
&=\int_{\delta_1=0}^\infty f_1(\delta_1)F_2(\delta_2)\;d\delta_1\\
&\leq\int_{\delta_1=0}^d f_1(\delta_1)F_2(\delta/(\delta_1+1))\;d\delta_1 + F_1(\delta)\\
&=\exp(-\mu\delta^2)+\int_{\delta_1=0}^d \left(2\mu\delta_1 \exp(-\mu(\delta_1^2+(\delta/(1+\delta_1))^2)\right)\;d \delta_1\\
&\leq\exp(-\mu\delta^2)+2\mu\delta \int_{\delta_1=0}^d \exp(-\mu(\delta_1^2+(\delta/(1+\delta_1))^2)\;d \delta_1
\end{align*}
We now want to know the minimal
value of 
$\delta_1^2+(\delta/(1+\delta_1))^2$. By 
differentiation, this is when 
\[2\delta_1-2\delta^2/(1+\delta_1)^3=0\iff
\delta_1(1+\delta_1)^3=
\delta^2.\]
In particular, $\delta_1<\delta^2$, so if
$\delta=o(1)$, then $\delta_1=o(\delta)$ and $\delta_2=\delta/(1+\delta_1)\sim\delta$. For $\delta=1$, this implies $\delta_1\leq 0.4$.

Perhaps I did the above way too complicated. Being a bit less precise, we can just
distinguish between the case
$\delta_1\geq \delta$, and the
case $\delta_1\leq\delta$, which for $\delta=o(1)$ again implies $\delta_2\sim \delta$, that is, for smaller $\delta$, we can just use
the union bound that
\[\Pr[X\leq \E[X]-\delta \mu]=F(\delta)<F_1(\delta)+F_2(\delta/(1+\delta)).\]




\drop{


\paragraph{Even better but also more tricky}
Basic idea is that the smaller a bound $\mu^+$, we have on the number
$X$ of selected keys, the better a bound $\mu^+_{\leq k}$ we get
on each $X_{\geq} k$ when we distribute the selected keys fully
randomly in buckets. Currently, we use a high probability
bound $\mu^+$ on $X$, but lets instead use
\[\mu^+=\mu+\sqrt{3\mu}.\]
By our Chernoff upper tail bound,
\[\Pr[X>\mu^+]<1/e\]
Analyzing Experiment 1, using a smaller $\mu^+$, we can derive
a smaller concrete value $\mu^+_{\geq k}$
and a concrete small probability bond $P_{\geq k}$,
\[\Pr[X_{\geq k}>\mu^+_{\geq k}\mid X\leq\mu^+]\leq P_{\geq k}.\]

In Experiment 2, after first part, define
\[Y_{\geq k}=\E[X_{\geq k}].\]
Now $Y_{\geq k}$ fixed for the last part of Experiment 2. In
this last part, $X_{\geq k}$ is settled as
a sum of independent 0-1 variables. By Chernoff, with
$\delta=\sqrt{2/Y_{\geq k}}$ and
\[Y_{\geq k}-=(1-\delta)Y{\geq k}=Y{\geq k}-\sqrt{2Y{\geq k}}\textnormal,\]
we get
\[\Pr[X_{\geq k}\leq Y^-_{\geq k}]\leq \exp(-\delta^2Y/2)=1/e.\]
The important thing is that this holds regardless of the value of $Y_{\geq k}$.

To connect to the $P_{\geq k}$ from Experiment 1,
we note that
\begin{align*}
  \Pr[X_{\geq k}> \mu^+_{\geq k}\mid X\leq\mu^+]&\geq\Pr\left[[X_{\geq k}>Y^-_{\geq k}>\mu\
^+_{\geq k}]\mid X\leq\mu^+\right]\\
&=\Pr\left[Y^-_{\geq k}>\mu^+_{\geq k}\mid X\leq\mu^+\right]\\
  &\quad\cdot \Pr\left[[X_{\geq k}>Y^-_{\geq k}\mid Y^-_{\geq k}>\mu^+_{\geq k}]\mid X\leq\
\mu^+\right]\\
\end{align*}
Here
\begin{align*}
  &\Pr\left[[X_{\geq k}>Y^-_{\geq k}\mid Y^-_{\geq k}>\mu^+_{\geq k}]\mid X\leq\mu^+\right]\\
  &\geq 1-\Pr\left[[X_{\geq k}\leq Y^-_{\geq k}\mid Y^-_{\geq k}>\mu^+_{\geq k}\right]+
    \Pr\left[X>\mu^+\right]\\
  &\geq 1-2/e.
\end{align*}
Thus we conclude that
\[\Pr[Y_{\geq k}-\sqrt{2Y_{\geq k}}>\mu^+_{\geq k} \mid X\leq\mu^+]\leq P_{\geq k}/(1-2/e)\
.\]
Here the conditioning is fine since we are trying to prove an upper bound
on the probability that $X<(1-\delta)\mu$ which can only be helped by the condition,
that is, 
\[\Pr[X<(1-\delta)\mu]=\Pr[X<(1-\delta)\mu\mid X\leq \mu^+]/\Pr[X>\mu^+]
\leq \Pr[X<(1-\delta)\mu\mid X\leq \mu^+]/e.\]
Now, we we condition on  $X\leq \mu^+$,
we get the above high probability
bounds that $Y_{\geq}\leq \mu^+_{\geq k}$.
If we in the last step ignore the
condition that $X\leq \mu^+$, then, as
usual, we have independent random
variables deciding the $X_a$ and hence
the sum. The sum is well concentrateed, and the probability that it exceeds $\mu^+$ is bounded by a constant. Hence,
the conditioning can only increase the
probability that $X<(1-\delta)\mu$ by a constant.

All in all, I think this idea gets a bit too complicated. Perhaps better just to accept some slightly worse constant
using a high probability bound $\mu^k$ on $X$, allowing us to do the analysis more independently.

}



\paragraph{Now back to what I had written}

We analyze by considering two different random experiments
fixing the same things, but in different order.

We are aiming of some bounds
that are of the form 
\[\Pr[X<(1-A\delta)\mu]\leq 
B\exp(-\mu\delta^2/C)+7\mu^3(3/\size\Sigma)^d.\]
Note that the first term dominates the usual $1/2^{\size\Sigma/2}$.
We will actually have some pretty small constants $A$,  $B$, and $C$ though I didn't optimize them yet. I shall refer to impact on these constants below.

\paragraph{The first experiment}
The basic idea is that we to first first fix the last character table
for the $d$'th derived character. Then the randomness is only from the hash
values we get from the tornado of the derived key minus the last
character. These hash values are from $\Sigma\times\cR$.  Based on the
fixed last character table, we get a modified selection function that
besides the usual select bits use the last character value.

If the query set is of at most one key, then the fixing of the last
table does not affect the expected number of selected keys since the
hash values are still 2-indendent. Below, for simplicity, we forget
about the query key.

Thus we still have the same expectation $\mu \leq \size\Sigma/2$.
By our main theorem, w.h.p, ( $(3/\size\Sigma)^{d-3}$ instead of
$(3/\size\Sigma)^{d-2}$, but that is OK), the keys are linearly
independent. In particular, we can apply
our clean Chernoff upper tail bound from \Cref{lemma:upper-chernoff}.
All the bounds are
based on events in conjunction with linear independence of the original
selected keys which is a joint
event for all applications of \Cref{lemma:upper-chernoff}), and for short we refer to them
as \emph{and-probabalities}. In particular, we can do this when we
futher select on the value of the last character being in a
set of $k$ given charater values.

Define $f=\mu/\size\Sigma$. We have assumed $f\leq 1/2$. Also,
define $\ell=\size\Sigma/k$, ignoring if this is not an integer.

We can pick $k$ characters
in $\binom{k\ell}{k} < (e\ell)^k$ ways. The
expected number of keys being selected based on a conrete
choice of the $k$ characters is $fk$. By \Cref{lemma:upper-chernoff},
the and-probability of getting
$K=(1+\delta)kf$ keys is bounded by
\begin{equation}\label{eq:error-prob-K}
  (ekf/K)^K
\end{equation}
We want this to be at least the square of $1/(e\ell)^k$, that is,
\[(K/ekf)^K\geq (e\ell)^{2k}\]
Our purpose is to say that we can have at most
at most $k$ buckets \lb{Here bucket means the set of keys selected by a given $d$-th character, so that there are $|\Sigma|$ buckets in total, I guess.}\mt{yes} with more than $K/k$ keys and we refer to this
quantity as the min-size. For some paramenter $\eps\leq\eps_0\leq 1/4$ to
be decided, we fix \lb{I got a bit lost with this new parameterization. It seems like this implies $\eps = (1+\delta) / \ell$}
\begin{equation}\label{eq:fix-K}
  K=\eps\mu=\eps fk\ell.
  \end{equation}
Then our error probability from \req{eq:error-prob-K} becomes \lb{This should be equivalent to $(e / (1+\delta))^{(1+\delta) fk}$}
\begin{equation}\label{eq:error-prob-ell}
(e/\eps\ell)^{\eps fk\ell}
\end{equation}
To get this bigger than $(e\ell)^{2k}$,
we need
\begin{equation}\label{eq:prob-dom-combi}
(\eps\ell/e)^{\eps f\ell/2}\geq e\ell.
\end{equation}
\lb{Or equivalently, we need $((1+\delta) / e)^{(1+\delta) f} \geq e \ell$. Hence, $\delta = \Omega(\log \ell / \log \log \ell)$, for constant $f$.}
and this should hold for any $\eps\leq 1/4$. 

Note however, that by \req{eq:fix-K}, the  
min-size of a bucket size is
\begin{equation}\label{eq:min-bucket-K}
  K/k=\eps f\ell.
\end{equation}
and for $\eps=1/4$, we want the min-size to be $O(1)$,
that is
\begin{equation}\label{eq:limit-first-buckets}
  f\ell=O(1).
  \end{equation}
It appears we solve both \req{eq:limit-first-buckets} and \req{eq:prob-dom-combi} by setting
\begin{equation}\label{eq:fix-ell}
\ell=8/(f\eps^{7/6})
\end{equation}
\mt{The $\eps^{7/6}$ will be important later. I am not sure that 8 is correct, 
and we should try to make it as small as possible since it goes straight into the constant $C$ in our bound.}

With this fix of $\ell$, the min-size becomes
\begin{equation}\label{eq:max-bucket-K}
  \eps f\ell=8/\eps^{1/6}.
\end{equation}
Recall that \req{eq:prob-dom-combi} ensured that the
the error probability from \req{eq:error-prob-ell} was
the square of the the inverse of the number of ways the $k$
characters could be picked, so union bounding over all
cases, we get a total error probability of
\begin{equation}\label{eq:error-prob-f}
  (e/\eps\ell)^{\eps fk\ell/2}=(\eps^{1/6} f/8)^{\eps \mu/2}
  <(f/8)^{\eps \mu/2}.
\end{equation}
This is the error probability for the first experiment. It will be
dominated by error probabilities from the second experiment.

To be a bit more precise,
we do not need to consider
an $\eps\leq \delta^2/2$. The  point is that with
$\eps\leq \delta^2/2$, we are bounding
the probability of getting more then $\eps\mu=
\delta^2\mu/2$
keys selected by
characters selecting more
than $8/\eps^{1/6}$
keys. It is OK
if we loose this many,
\mt{costs a factor $(1+\delta)$ in $A$}
and 
$f/8\leq 1/16<1/e^2$, so 
\begin{equation}\label{eq:good-error-bound}
(f/8)^{\eps \mu/2}<
\exp(-\mu\delta^2/2).
\end{equation}

\lb{Anyhow, let's assume for now that the union bound over all possible $k$-tuples work and we are ensured that there exists no $k$-tuple of characters $(\sigma_1 \dots \sigma_k)$ such that for each $\sigma_i$ there are $K/k = (1+\delta) f$ keys that are selected and have $\sigma_i$ as their last character.}


\paragraph{Partitioning bucket into levels}
We are going to define some levels $i=1,2\ldots$.
we define $\eps_i=1/2^{i+1}$. Then the min-size
defined above is below $m_i=8/\eps_i=8/2^{(i+1)/6}$. \lb{According to your definition of $\eps_i$, the last equality seems false. I just assume $m_i := 8/2^{(i+1)/6}$}
We also define $m_0=1$. Finally, for $i=0,1,2\ldots$.
we define $X_i$ be the total number of keys
selected for by character buckets of size in the range
$[m_i,m_{i+1})$. Then the total set $X$
  of selected keys in the union of the $X_i$ since
all bucket sizes are considered.

Assume that the first experiment succeeded for all $\eps_i$, $i\geq 1$. Then
we know that the total number of keys landing in character selected
buckets with at
least $m_i$ keys is $<\eps_i\mu$. In particular this implies
that $\size {X_i}<\eps_i\mu$.

Let $i_{\max}$ be the largest
value of $i$ such that $\eps_i>\delta_i/2$ We will
not consider $i>i_{\max}$, since
we already saw that if the first experiment succeeded,
then there are so few keys
belonging to higher levels that we can afford to loose all of them.

Note that the total error
probability over all levels
is 
\[\sum_{i=1}^{i_{\max}}(f/8)^{\eps_i\mu/2}.\]
The last term dominates strongly since the $\eps_i$ 
are proportional to $1/2^i$.
But we already saw in
\req{eq:good-error-bound}
that the last term was
dominated by 
\[\exp(-\mu\delta^2/2).\]


\paragraph{Second experiment}
We now want to consider the above experiment where we fix the
table for the last derived character last.
Suppose everything else has been fixed first. When we now fix the hash
of one character from the last table, then this fixes which keys
keys we get with this last derived character. If the number
falls in $[m_i,m_{i+1})$ then they constribute to $X_i$ as defined
above.

When all other character tables were fixed first, then the numbers from
different last characters are completely independent. If follows
that each $\size {X_i}$ is the sum of independent random variables
that are either $0$ (when a character did not contribute to $X_i$) or
$[m_i,m_{i+1})$. In particular, they are all below $m_{i+1}$.

So far we have an unkown expectation $\mu_i=\E[\size X_i]$ whose
value depends on the how we fixed all first character tables.
However, we do know that $\sum_i\mu_i=\mu$, and by Chernofff, for any $\delta_i\in(0,1]$, 
\[\Pr[\size {X_i}<(1-\delta_i)\mu_i]\leq \exp(-(\mu_i/m_{i+1})\delta_i^2/2).\]
We do not known $\mu_i$, but for other reasons (to be explained later),
we can insist that
\begin{equation}\label{eq:not-to-small}
  (\mu_i/m_{i+1})\geq 8\textnormal,
\end{equation}
\lb{If this bounds is derived from your definition of $m_i = 8 / \eps_i$ then this contradicts $m_i = 2^{(i+1) / 6}$.}
In particular it follows that 
\[\Pr[\size {X_i}<\mu_i/2]\leq 1/e.\]
\mt{We should be able
to loose much less than
a factor $2$. Is there
a theorem saying that if
we sum independent variables
below 1, then with probability 1/2, we do get something below expectation minus $1$??}

Thus, if $\mu_i\geq 2\eps_i\mu$, then
\[\Pr[\size {X_i}>\eps_i\mu]\geq (1-1/e)>1/2.\]
Thus, if for any $i$, we have $\mu_i\geq 2\eps_i\mu$,
then the probability that got a violation of the first experment
that created the same event is at least  $1/2$. We  conclude
conversely the probability of any such event after just fixing
all but the last character tables is at most twice
the error probability for all levels for the the first experiment.

We assume that this didn't happen when fixing all but the last table.
Then we know $\mu_i\leq 2\eps_i\mu$ and therefore 
\[\Pr[\size {X_i}<\mu_i-\delta_i 2 \eps_i \mu]\leq
\exp(-(2 \eps_i \mu/m_{i+1})\delta_i^2/2).\]
This is for $i>0$, but we also know that $\mu_0\leq\mu$, so
\[\Pr[\size {X_0}<\mu_0-\delta_0 \mu]\leq
\exp(-(\mu\delta_0^2/2).\]
If none of the above errors happen, then
\[X>(1-\delta-2\sum_{i=0}^{i_{\max}}\delta_i\eps_i)\mu\]
All that remains is to pick the $\delta_i$ such that
$\sum_{i=0}^{i_{\max}}\delta_i\eps_i=O(\delta)$ and such that
the total error probability is
$\exp(-\Omega(\mu\delta^2))$. We chose
\[\delta_i=\delta 2^{2(i+1)/3}\]
The rest is simple calculations. We have
\[2\sum_{i=0}^{i_{\max}}\delta_i\eps_i<2\delta\sum_{i=0}^{\infty} 2^{2(i+1)/3}/2^{i+1}=
\frac{2^{4/3}}{1-2^{1/3}}\delta
<12.3\delta.\]
We have to include the original $\delta$ plust the $\delta^2/2$ we have gave up
from the levels above $i_{\max}$, so
if none of our errors happen, then 
\[X>(1-14\delta)\mu.\]
\mt{So $B=12$.. was hoping for smaller, but still not crazy}

For the error probabilities, we now have \lb{I cannot follow these computations, it seems like you replaced $\eps_i$ with $2^{i+1}$ rather than $2^{-(i+1)}$ and  $m_i$ with $8 / 2^{(i+1) / 6}$. All in all, it seems like $\eps_i$ being small helps the bound rather than being a hurdle.} 
\[\exp(-(2\eps_i\mu/m_{i+1})\delta_i^2/2)=
\exp(-2 \mu 2^{i+1}/(8/2^{(i+1)/6}))(\delta 2^{2(i+1)/3})^2/2)
=\exp(-\mu \delta^2 2^{(i+1)/6})/16)\]
This falls quite quickly, so our error probability for
the whole sums is probably below
\[\exp(-\mu\delta^2/8)\]
\mt{Again an important constant to compute}
\paragraph{Better for small expectations (very sketchy)}
If selection is done by 
a simple bit map, and we have a small $\mu$, then we
can do the usual trick of first freeing some bits to
get a $\mu'$ close to $\size\Sigma/2$, and then subsample refixing the bits enjoying full randomness. \lb{Seems like it should work.}

\lb{All in all, I understood the main ideas (very nice proof :D). However, I am not sure the computations work. Most likely they do, but I cannot follow them as they're here.}
\mt{These were just some quick initial calculations.. As I now hinted in the beginning of the section, I think we can do something far tighter via second moments and Bernstein's inequality}


==> Notes/jonasTODO.tex <==
\section{Jonas' TODO's}
\begin{itemize}
\item Editing proofs:
\begin{itemize}
    \item Fix parameter names, in statements, proofs and arguments
    \item Fix \(\calI\) to new notation
\end{itemize}
\item Presentation of main results
\begin{itemize}
    \item Unpack gamma1, rename gamma2 to eps, if we want to present technical theorem
    \item Figure out inclusion/exclusion of event \(\calI\)
    \item Reconsider type (theorem/lemma/corollary) of main statements.
\end{itemize}
\item Improve readability of proof of \cref{lem:topLayers_2}.
\item Improve readability of proof of \cref{thm:pretty1}
\end{itemize}

\section{Jonas' DONE's}
\begin{itemize}
\item Define \(p_i\)'s, layer types and their relation to the messy table.
\begin{itemize}
    \item Clean up list of symbols, and rename 'c' to avoid conflict with ``number of characters'' used for tabulation hashing.
    \item Define \(p_i\)'s.
    \item Describe symbols of table
\end{itemize}
\item Proof of lem:layer-size-chernoff (including non-indep Chernoff in Appendix)
\item Proof of lem:conditionalTranslation
\item Proof of prettySubsampling, independent of old pretty-theorem (now junked)
\end{itemize}


==> Notes/jonasnotes.tex <==
\section{Jonas' Sandbox}
\subsection{The Poisson connection}
\begin{lemma}
  Let \(X_1, \dots, X_{\ssigma}\) be \(\{X_\alpha\}_{\alpha \in \Sigma}\) sorted in non-increasing order.
  For any \(k = 1, \dots, \ssigma\) and \(q \in \mathbb N\)
  \[
  \Prp{\sum_{i=1}^k \size{X_i} \geq q \land \calI} \leq \binom{\ssigma}{k} \cdot \binom{n}{q} \cdot \left(\frac{k p}{\ssigma}\right)^q \leq \binom{\ssigma}{k} \cdot \frac{(kf)^q}{q!} \, .
  \]
\end{lemma}
Define \(S_i = \size{ \set{ X_\alpha \, : \, \size{X_\alpha} \geq i }}\) for \(i = 0, 1, 2, \dots\).
\begin{lemma}
  \[
  \Prp{S_i \geq k \land \calI} \leq \binom{\ssigma}{k} \cdot \binom{n}{i}^k \cdot \left(\frac{p}{\ssigma}\right)^{i\cdot k} \leq \binom{\ssigma}{k} \cdot \left(\frac{f^i}{i!}\right)^{k}
  \]
\end{lemma}

Let \(Z\) be a random variable distributed according to a Poisson distribution with mean \(f\) -- that is, \(\Prp{Z = k} = f^k/(k! e^f)\).
Then
\[\Prp{S_i \geq k \land \calI} \leq \binom{\ssigma}{k} e^f \Prp{Z = i}^k \leq \binom{\ssigma}{k} e^f \Prp{Z \geq i}^k \, .\]

Let \(Q(R) = \set{\min k \in \mathbb Z : \Prp{Z \leq k} \geq R}\) be the quantile function for the distribution of \(Z\).
Then \(Q(1-p)\) is the smallest integer \(k\) s.t. \(\Prp{Z > k} < p\).
Let \(\Phi^{-1}\) be the ``probit'' function, the quantile function of the normal distribution.
\begin{lemma}[Discussed in \cite{bailey1981alternatives,short2013improved}, originally from \cite{hastings1955}?]
  \[
  \Phi^{-1}(R) \leq \sqrt{-2 \cdot \ln(2 \cdot (1-R))} \, .
  \]
\end{lemma}
\begin{lemma}[\cite{short2013improved}, Theorem 4]
  For \(R \in [0.5, 1)\)
    \[
    Q(R) \leq \ceil{f + \Phi^{-1}(R) \sqrt{f} + \frac{\Phi^{-1}(R)^2}{6}} \, .
    \]
\end{lemma}


\subsection{Bounding max}
We want to find a value \(\tau\) s.t. \(\Prp{\max \size{X_\alpha} > \tau} \leq \exp(c)\) for a value \(c\) to be settled later.

\begin{lemma}
  \[\Prp{ \max_{\alpha \in \Sigma} \size{X_\alpha} \land \calI > \ln(\ssigma) - \frac{2c}{3}} < \exp(c) \]
  For \(c \leq -6\).
\end{lemma}
\begin{proof}
  Let \(d = c - \ln(\ssigma) - f\) and \(\tau = Q(1-\exp(d))\).
  \begin{align*}
    \tau &\leq \ceil{f + \Phi^{-1}(1-\exp(d)) \sqrt{f} + \frac{\Phi^{-1}(1-\exp(d))^2}{6}} \\
    &\leq \ceil{f + \sqrt{-2 \cdot \ln(2 \cdot \exp(d))} \sqrt{f} + \frac{-2 \cdot (\ln(2) + d)}{6}} \\
    &\leq \ceil{f-0.23 + \sqrt{-2 \cdot \ln(2 \cdot \exp(d))} \sqrt{f} - \frac{d}{3}} \\
    &\leq \ceil{f-0.23 - \frac{2d}{3}} & \text{For \(d \leq -8.5\), and using \(f \leq 1/2\)} \\
    &\leq \ceil{f-0.23 + 2 \cdot \frac{\ln(\ssigma) + f - c}{3}} \\
    &\leq \ln(\ssigma) - \frac{2c}{3} & \text{for \(\ln(\ssigma) \geq 2.5\).} \\
  \end{align*}

  \begin{align*}
    \Prp{ \max_{\alpha \in \Sigma} \size{X_\alpha} > \ln(\ssigma) - \frac{2c}{3} \land \calI } &\leq \Prp{ \max_{\alpha \in \Sigma} \size{X_\alpha} > \tau \land \calI} \\
    &\leq \ssigma \cdot \Prp{\size{X_\alpha} > \tau \land \calI} \\
    &\leq \ssigma \cdot e^f \Prp{Z > \tau} \\
    &\leq \ssigma \cdot e^f \exp(d) \\
    &= \ssigma \cdot e^f \exp(c - \ln(\ssigma) - f) \\
    &= \exp(c) \, .
  \end{align*}
\end{proof}

\subsection{Sum of squares}
\begin{observation}
  \[
  \sum_{\alpha \in \Sigma} \size{X_\alpha}^2 = \sum_{i=1}^\infty i^2 \cdot \size{\set{X_\alpha \, | \, \size{X_\alpha} = i}} = \sum_{i=1}^\infty i^2 \cdot (S_i - S_{i+1}) = \sum_{i=1}^\infty (i^2 - (i-1)^2) S_i = \sum_{i=1}^\infty (2i-1) S_i \, .
  \]
\end{observation}
\begin{lemma}
  \[ \Ep{\sum_{\alpha \in \Sigma} \size{X_\alpha}^2 \land \calI} \leq 2 \mu \, . \]
\end{lemma}
\begin{proof}
  \begin{align*}
    \Ep{\sum_{\alpha \in \Sigma} \size{X_\alpha}^2 \land \calI} &= \sum_{\alpha \in \Sigma} \sum_{k = 1}^\infty (2k-1) \Prp{\size{X_\alpha} \geq k \land \calI} \\
    &\leq \ssigma \sum_{k=1}^\infty (2k-1) \cdot \frac{f^k}{k!} \\
    &= \mu \sum_{k=1}^\infty (2k-1) \cdot \frac{f^{k-1}}{k!} \\
    &\leq \mu \sum_{k=1}^\infty (2k-1) \cdot \frac{1}{k! 2^{k-1}} \\
    &= \mu \sum_{k=1}^\infty \frac{2k}{k!2^{k-1}} - \frac{1}{k!2^{k-1}} \\
    &= \mu \sum_{k=1}^\infty \frac{1}{(k-1)!2^{k-2}} - \frac{1}{k!2^{k-1}} \\
    &= \mu \cdot \frac{1}{0!2^{-1}} = 2\mu & \text{(telescoping sum).}
  \end{align*}
\end{proof}

\subsection{Bounding a squared sum through bounds on prefix-sums (discarded approach)}
\begin{lemma}
  Let \(x_1 \geq x_2  \geq \dots \geq x_d \geq 0\) be positive reals and \(n_1, \dots, n_d\) be chosen such that \(\sum_{i=1}^q x_i \leq n_q\) for \(q = 1, \dots, d\).
  Define \(z_1 = n_1\) and \(z_q = n_q - n_{q-1}\) for \(q = 2, \dots, d\).
  Then
  \[
  \sum_{i=1}^d x_i^2 \leq \sum_{i=1}^d z_i^2 \, .
  \]
\end{lemma}

\begin{proof}
  Define \(\Delta_q = n_q - \sum_{i=1}^q x_i \geq 0\) for each \(q = 1, \dots, d\).
  We prove the following claim: For each \(q = 1, \dots, d\), \(\sum_{i=1}^q z_i^2 - x_i^2 \geq 2x_q\Delta_q\).

  The claim is true for \(q=1\) as \(z_1^2 - x_1^2 = (x_1 + \Delta_1)^2 - x_1^2 = \Delta_1^2 + 2x_1\Delta_1\).
  For \(q>1\) we have
  \[z_q = n_q - n_{q-1} = \sum_{i=1}^q x_i + \Delta_q - \parentheses{\sum_{i=1}^{q-1} x_i + \Delta_{q-1}} = x_q + \Delta_q - \Delta_{q-1} \, .\]
  Assuming the claim holds for \(q-1\) we get
  \begin{align*}
    \sum_{i=1}^q z_i^2 - x_i^2 &= \parentheses{\sum_{i=1}^{q-1} z_i^2 - x_i^2} + z_q^2 - x_q^2 \\
    &\geq 2x_{q-1} \Delta_{q-1} + (x_q + \Delta_q - \Delta_{q-1})^2 - x_q^2 \\
    &= 2x_{q-1} \Delta_{q-1} + (\Delta_q - \Delta_{q-1})^2 +2x_q\Delta_q - 2x_q \Delta_{q-1} \\
    &= 2x_q\Delta_q + 2\Delta_{q-1}(x_{q-1} - x_q) + (\Delta_q - \Delta_{q-1})^2 \\
    &\geq 2x_q\Delta_q \, ,
  \end{align*}
  where the last inequality uses that \(x_{q-1} \geq x_q\).
\end{proof}

\subsection{Using point probabilites for better bounds}

\begin{observation}
  \[\Prp{S_i < \Epcond{S_i}{\barh} - t} = \sum_{k=0}^\infty \Prp{\Epcond{S_i}{\barh} = k} \cdot \Prpcond{S_i < \Epcond{S_i}{\barh} - t}{\Epcond{S_i}{\barh} = k} \]
\end{observation}
\begin{proof}[Comments]
  The second part (``error2'') we already know how to approach, but calculating the point-probabilities of \(\Epcond{S_i}{\barh}\) (``error1'') seems infeasible.
  Perhaps we can show that the ``worst-case'' distribution of \(\Epcond{S_i}{\barh}\) is the one that follows Chernoff-bounds exactly, in which case Mikkel's calculations suggest that the terms with \(k \approx \Ep{S_i}\) will by far be the most expensive ones.

  \st{Something is fishy, though.} As small \(k\) makes error2 very probable -- I find it difficult to believe that all of these cases could be wrapped up in the term \(k=\Ep{S_i}\), which is where Chernoff would start off (?).
  Part 1 is most probable centered around \(k=\Ep{S_i}\) while (2) is decreasing in \(k\).

  Fix is that we consider an \emph{absolute} deviation. Absolute deviation only becomes more likely with higher conditional expectation -- which in turn are less likely. The two can then hopefully balance out.
\end{proof}


\subsection{2 layers with Bernstein}
\begin{lemma}[2 layers with Bernstein]\label{lem:2layers}
  Assume that \(\ln(1/p) \leq \ssigma f^2/6 = \bar \mu_2  /3\).
  
  Let \(\mu' = \left(1 + \sqrt{6 \ln(1/p)/\ssigma}\right) \mu + 2 \approx \mu\) and
  \(t = \sqrt{2\ln(1/p) \left(\mu' + \frac{2}{9} \ln(1/p) \right) } + \frac{2}{3} \ln(1/p) \approx \sqrt{2\ln(1/p)\mu} . \)
  Then
  \[ \Prp{(S_1 + S_2) \leq \Epcond{S_1 + S_2}{\barh} - t} \leq 3p \, . \]
\end{lemma}
\paragraph{Proof}
Bernstein's inequality for independent non-centered variables \(\size{X_i} \leq M\) states
\[\Prp{\sum X_i \leq \Ep{\sum X_i} + t} \leq \exp\left( \frac{- 0.5 t^2}{\sum \Var[X_i] + t \cdot M/3} \right) \, .\]
Let \(\bar X_\alpha = \min\set{2, \size{X_\alpha}}\).
As \((S_1+S_2) = \sum_\alpha \bar X_\alpha\), which are independent when conditioned on \(\barh\),
  \[\Prpcond{S_1 + S_2 < \Epcond{S_1+S_2}{\barh} - t}{\barh} \leq \exp\left(\frac{-0.5t^2}{\sum_{\alpha\in\Sigma} \Varcond{\bar X_\alpha}{\barh} + t \cdot 2/3} \right) \, .\]

  Define \(\bar \mu = \sum_{\alpha} \Epcond{\bar X_\alpha}{\barh} = \Epcond{S_1+S_2}{\barh}\) and \(\bar f = \bar \mu / \ssigma\).
  It then holds that \(\sum_\alpha \left(\Epcond{\bar X_\alpha}{\barh}\right)^2 \geq \sum_\alpha (\bar \mu/\ssigma)^2 = \ssigma \bar f^2\) and thus
  \begin{align*}
    \sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} &= \sum_{\alpha \in \Sigma} \Epcond{\bar X_\alpha^2}{\barh} - \sum_{\alpha \in \Sigma} \left(\Epcond{\bar X_\alpha}{\barh}\right)^2 \\
    &\leq \sum_{\alpha \in \Sigma} \Epcond{\bar X_\alpha^2}{\barh} - \ssigma \bar f^2 \\
    &= \sum_{\alpha\in\Sigma} \Epcond{\bar X_\alpha(\bar X_\alpha - 1)}{\barh} + \sum_{\alpha\in\Sigma} \Epcond{\bar X_\alpha}{\barh}  - \ssigma \bar f^2 \\
    &= 2 \cdot \Epcond{S_2}{\barh} + \bar \mu - \ssigma \bar f^2 \, .
  \end{align*}
  We will now bound \(\Epcond{S_2}{\barh}\).
  Applying \cref{lem:layer-size-chernoff} with \(\delta = \sqrt{3 \ln(1/p)/\bar \mu_2} = \sqrt{6 \ln(1/p)/(f^2 \ssigma)}\) we have
  \[
  \Prp{S_2 \geq (1 + \delta) \ssigma f^2/2} \leq p \, .
  \]
  Invoking \cref{lem:conditionalTranslation}, we have for \(\mu^+ = (1+\delta)\ssigma f^2/2 + 1\)
  \[
  \Prp{\Epcond{S_2}{\barh} \geq \mu^+} \leq 2p \, .
  \]
  Hence, with probability at least \(1-2p\),
  \begin{align*}
    \sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} &< 2\mu^+ + \bar \mu - \ssigma \bar f^2 \\
    %% &\leq 2\cdot \Epcond{S_2}{\barh} + \bar \mu - \ssigma \bar f^2 \\
    &= (1+\delta) \ssigma f^2 + \bar \mu - \ssigma \bar f^2 + 2 \, .
    %% &\leq 2\left((1+\delta)\ssigma f^2/2 + \sqrt{(1+\delta) \ssigma f^2/2}\right) + \bar\mu - \ssigma \bar f^2
  \end{align*}
  Note that the function \(x \mapsto x-x^2\) is increasing in \(x \in [0, 1/2]\).
  As \(\bar f \leq f \leq 1/2\) we thus have \(\bar f - \bar f^2 \leq f - f^2\) and
  \[
  \ssigma f^2 + \bar \mu - \ssigma \bar f^2 = \ssigma (f^2 + \bar f - \bar f^2) \leq \ssigma \cdot f = \mu
  \]
  giving
  \begin{align*}
    \sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} &\leq \mu + \delta \ssigma f^2 +2 \\
    &= (1 + \delta f) \mu + 2 \, .
  \end{align*}
  Note that
  \begin{align*}
    \delta f &= f \sqrt{6 \ln(1/p) /(f^2 \ssigma)} \\
    &= \sqrt{6 \ln(1/p)/\ssigma}
  \end{align*}
  and thus \(\sum_\alpha \Varcond{\bar X_\alpha}{\barh}\) will be roughly \(\mu\) whenever \(\mu\) is large and \(\ln(1/p) \ll \mu\).
  
  In summary, we have the following guarantee on the conditional variance.
  \begin{lemma}
    If \(\ln(1/p) \leq \ssigma f^2/6 = \bar \mu_2/3\),
    \[\Prp{ \sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} >  \left(1 + \sqrt{6 \ln(1/p)/\ssigma}\right) \mu + 2 } < 2 p \, .\]
  \end{lemma}

  Conditioning on \(\sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} \leq \mu' = \left(1 + \sqrt{6 \ln(1/p)/\ssigma}\right) \mu + 2\), Bernstein's now gives
  \[\Prpcond{S_1 + S_2 \leq \Epcond{S_1+S_2}{\barh} - t}{\barh, \, \sum_{\alpha \in \Sigma} \Varcond{\bar X_\alpha}{\barh} \leq \mu'} \leq \exp\left(\frac{-0.5t^2}{\mu' + t \cdot 2/3} \right) \, .\]
  Solving for \(t\) we find
  %% Solve: https://www.wolframalpha.com/input?i2d=true&i=Divide%5B0.5Power%5Bx%2C2%5D%2Ca%2BDivide%5B2x%2C3%5D%5D%3Dc
  \begin{align*}
    &t \geq \sqrt{2\ln(1/p) \left(\mu' + \frac{2}{9} \ln(1/p) \right) } + \frac{2}{3} \ln(1/p) \\
    \implies &\exp\left(\frac{-0.5t^2}{\mu' + t \cdot 2/3} \right) \leq p \, .
  \end{align*}

  Including the probability that \(\sum_\alpha \Varcond{\bar X_\alpha}{\barh} > \mu'\), \cref{lem:2layers} follows.

\subsection{Regular layers from 3}
\begin{lemma}[Sum of regular layers, starting at 3]\label{lem:regularLayers3}
  \[\Prp{\sum_{i=3}^{i_0 - 1} S_i \leq \Epcond{S_i}{\barh} - \Delta} \leq (i_0-3) \cdot 3p\]
  where \(\Delta = 0.614 \sqrt{\ln(1/p) \mu} + (i_0 - 3) \sqrt{2\ln(1/p)}\).
\end{lemma}
\begin{proof}
  Note that \(0.614 \sqrt{\mu} \geq \sqrt{1+\sqrt{3}\cdot\mu/12} \geq \sqrt{2 (1+\sqrt{3})\bar \mu_3}\). Thus \(\Delta \geq \Delta_3\), as defined in \cref{lem:regularLayer}, and if \(i_0 = 4\) the statement is true by a single application of the same lemma.

  Now assume \(i_0 > 4\). Then \(\ln(1/p) \leq \bar \mu_4 = \bar \mu_3 \cdot f/4\).
  Again referring to \cref{lem:regularLayer} we have
  \[\varepsilon_3 = \sqrt{3 \ln(1/p)/\bar \mu_3} \leq \sqrt{f \cdot 3/4} \leq \sqrt{3/8} \, .\]
  Summing over \(\Delta_i\) now gives
  \begin{align*}
    \sum_{i=3}^{i_0 - 1} \Delta_i &= \sqrt{2\ln(1/p)} \sum_{i=3}^{i_0 - 1} \sqrt{(1+\eps_i) \bar \mu_i + 1} \\
    &\leq \sqrt{2 \ln(1/p)} \cdot \left[ \sqrt{(1+\varepsilon_3) \bar \mu_3} + \sum_{i=4}^{i_0 -1} \sqrt{(1+\varepsilon_i) \cdot \bar \mu_i} + i_0 - 3\right] \\
    &\leq \sqrt{2\ln(1/p) \bar\mu_3} \cdot \left[ \sqrt{1+\varepsilon_3} + \sum_{i=4}^{i_0 -1} \sqrt{\frac{(1+\varepsilon_i)}{8} \cdot  \left(\frac{f}{5}\right)^{i-4}}\right] + (i_0 - 3) \sqrt{2\ln(1/p)} \\
    &\leq \sqrt{\ln(1/p) \mu/12} \cdot \left[ \sqrt{1+\sqrt{3/8}} + \sqrt{\frac{1+\sqrt{3}}{8}} \cdot \sum_{k=0}^{i_0 -5} \left(\frac{1}{\sqrt{10}}\right)^{k}\right] + (i_0 - 3) \sqrt{2\ln(1/p)} \\
    &\leq 0.614 \sqrt{\ln(1/p) \mu} + (i_0 - 3) \sqrt{2\ln(1/p)} \\
    %% SOLVE: https://www.wolframalpha.com/input?i2d=true&i=sqrt%5C%2840%291%2Bsqrt%5C%2840%29Divide%5B3%2C8%5D%5C%2841%29%5C%2841%29+%2B+sqrt%5C%2840%29Divide%5B%5C%2840%291+%2B+sqrt%5C%2840%293%5C%2841%29%5C%2841%29%2C8%5D%5C%2841%29*%5C%2840%29Sum%5BDivide%5B1%2CPower%5Bsqrt%5C%2840%2910%5C%2841%29%2Ck%5D%5D%2C%7Bk%2C0%2Cinfinity%7D%5D%5C%2841%29
  \end{align*}
  Hence
  \begin{align*}
    \Prp{\sum_{i=3}^{i_0 -1} S_i \leq \Epcond{S_i}{\barh} - \Delta} &\leq \sum_{i=3}^{i_0-1} \Prp{S_i \leq \Epcond{S_i}{\barh} - \Delta_i} \\
    &\leq (i_0 - 3) \cdot 3p \, .
  \end{align*}

  \subsection{Bounding layer size without Chernoff}
  \begin{lemma}[Bounding size of layer without Chernoff]
  \[\Prp{S_k \geq \frac{2e\ssigma f^k}{k!} \cdot \frac{\ln(1/p)}{\ln \ln(1/p)} \land \calI} \leq p \]
  when \(e \ssigma f^k/k! = e \bar \mu_k \geq 1\).
\end{lemma}
\begin{proof}[Proof sketch]
  Let \(q = \frac{2e\ssigma f^k}{k!} \cdot \frac{\ln(1/p)}{\ln \ln(1/p)}\).
  \begin{align*}
    \Prp{S_k \geq q \land \calI} &\leq \binom{\ssigma}{q} \cdot \left(\frac{f^k}{k!}\right)^q \\
    &\leq \left(\frac{e \ssigma f^k}{q \cdot k!}\right)^q \\
    &= \left(\frac{\ln \ln(1/p)}{2 \ln(1/p)}\right)^{q} \\
    &\leq \left(\frac{1}{\sqrt{\ln(1/p)}}\right)^{\frac{2\ln(1/p)}{\ln \ln(1/p)}} = p \, .
  \end{align*}
  Using that
  \[
  \frac{2 \log(1/p)}{\log \log(1/p)} = \frac{\log(1/p)}{\log \sqrt{\log(1/p)}} = \log_{\sqrt{\log(1/p)}}(1/p)
  \]
  for the final equality.
  The first inequality follows from the argument presented in the proof of \cref{lem:layer-size-chernoff} which bounds the probability that \(i\) chosen buckets are all large, combined with a union bound over all \(\binom{\ssigma}{q}\) choices of buckets.
\end{proof}

\end{proof}


==> Notes/poisson-notes.tex <==
\section{Jonas' notes on Poisson Sampling}
In Poisson Sampling we are given a set of elements \(S = \set{x_1, \dots, x_k}\) where each \(x_i\) has an associated weight \(p_i \in (0, 1]\).
We are tasked with sampling a subset \(X \subset S\) such that each \(x_i\) is included with probability \(p_i\), independently from the sampling of other elements.

With fully random hashing \(h^* \colon S \to \calR\) this is easily obtained by including \(x_i\) iff \(h(x_i) < p_i \cdot \size{\calR}\) (assuming that the \(p_i\) are all multiples of \(1/\size{\calR}\)).
With tornado tabulation \(h \colon S \to \calR\) it is less clear that this works at all, given the limited independence properties of tabulation hashing.

Informally, we establish that Poisson sampling, when implemented with tornado hashing, performs \emph{almost} as if implemented with fully random hashing, as long as the expected size of the sample is at most some fraction of \(\ssigma\).
Namely, the (distribution of the) number of sampled elements closely tracks the distribution obtained with full randomness.

For any set \(S\), we construct sets \(S^+\) and \(S^-\). Let \(X^+, X^-\) be the number of sampled elements from \(S^+, S^-\), respecively, using fully random hashing.
Let \(X\) be the number of elements sampled from \(S\) using tornado tabulation.
Further, we define a set of events \(\calE^+, \calE^-\).
We show that, when restricted to \(\calE^+\), \(X\) is stochastically dominated by \(X^+\).
Likewise, when restricted to \(\calE^-\), \(X\) dominates \(X^-\).
Formally, for all integers \(t \geq 0\),
\begin{align*}
  \Prp{X \geq t \land \calE^+} &\leq \Prp{X^+ \geq t \land \calE^+} \\
  \Prp{X \leq t \land \calE^-} &\leq \Prp{X^- \leq t \land \calE^-} \, .
\end{align*}
Borrowing the usual notation for stochastic dominance, we write this as \(X^- \preceq_{\calE^-} X \preceq_{\calE^+} X^+\).

These results are obtained, at a high level, by creating a specific coupling between \(X\) and \(X^+\), and defining event \(\calE^+\) on this joint distribution in such a way that \(\calE^+ \implies X \leq X^+\) (and symmetrically for \(X\) and \(X^-\)).

For these guarantees to be of any use, we need to ensure that \(\calE^+\) and \(\calE^-\) happen with high probability.
These events are used to mask extreme outcomes of the distributions and \(\neg\calE^+, \neg\calE^-\) can intuitively be viewed as a pair of error-events where no guarantees are made.
Further, the sets \(S^+\) and \(S^-\) should closely resemble \(S\), such that the distributions of \(X^+, X^-\) doesn't deviate much from the distribution of fully random poisson sampling of \(S\).
Specifically, \(S^+\) will be obtained by adding extra elements to \(S\), while \(S^-\) is obtained by removing elements from \(S\).
The number of elements added/removed, and thus the gap between the distribution of \(X^-\) and \(X^+\), will be parameterized by \(\ssigma\) and an adjustable probability of either error-event happening.

\subsection{Dominating Sets}
For two sets of elements \(A, B\) where elements of \(A\) have weights \(p_i\) and elements of \(B\) have weights \(q_i\) we say that \(A\) is \emph{dominated by} \(B\) if each \(p_i\) can be matched to a unique \(q_j\) such that \(p_i \leq q_j\).
An equivalent definition is that, for every threshold \(t \in [0, 1]\), the number of \(p_i\) greater than \(t\) is smaller than the number of \(q_i\) greater than \(t\).

Domination forms a partial order relation on sets of elements and we write \(A \leq B\).
Observe that dominance is closely related to stochastic dominance:
If \(A'\) and \(B'\) are the number of samples obtained by Poisson Sampling from \(A\) and \(B\), then \(A'\) is stochastically dominated by \(B'\) when \(A \leq B\).

We extend the partial order to ordered families of sets in a straightforward manner, such that \((A_1, A_2, \dots) \leq (B_1, B_2, \dots)\) iff \(A_i \leq B_i\) for all \(i\).

We will use this partial order in our arguments regarding stochastic dominance.
Hence \(A \preceq_\calE B\) denotes that, for all families of weighted sets \(T\),
\[\Prp{A \geq T \land \calE} \leq \Prp{B \geq T \land \calE} \, .\]

%% Abandoned, concepts didn't feel appropriate for general definition after all
%% \subsection{Subselection}
%% For selector functions \(f\) and \(f'\) (see definition in \cref{sec:prelim}), we say that \(f'\) is a subselector of \(f\) if the selection bits \(b'\) of \(f'\) is a superset of the selection bits \(b\) of \(f\), and \(f(x, r) = 0 \implies f'(x, r) = 0\).
%% Further, for each pair \((x, r)\) the value of \(f'(x, r)\) must be computable just by observing \(f(x, r)\) and the value of selection bits \(b' \setminus b\).
%% In other words, \(f'\) observes more selection bits and uses these to select a subset of the elements selected by \(f\).

%% If \(X'\) is the set of elements selected by \(f'\) and \(X\) the set of elements selected by \(f\) we will likewise say that \(X'\) is a subselection of \(X\).

%% \subsection{Dominance and Subselection}
%% In our proof we will perform a sequence of selections, where each selection is the union of (1) a subselection of the previous selection and (2) a selection on a new set of keys not considered before.

%% Notation quickly gets messy, as we are always comparing two experiments, one where keys are assigned hashvalues (and thus selected based on) tornado tabulation, and a separate experiment where the same process is carried out based on fully independently assigned hashvalues, but on a slightly larger (or smaller) set of elements.

%% Let us first describe the experiment based on tornado tabulation.
%% \(S\) is a set of elements parittioned into sets \((S_1, \dots, S_k)\) and \(f\) is a selector function, with the added property that \(f(x, \cdot) = f(y ,\cdot)\) for any \(x, y\) in the same partition.
%% For each \(i\) let \(A_i\) be the set of elements selected from \(S_i\), with hashvalues assigned by tornado tabulation.

%% Now, let \(f'\) be a subselector of \(f\), defined on a larger set \(S \cup S_{k+1}\), with the same restriction 
%% Let the elements selected by \(f'\) be \(A_1', \dots, A_{k+1}'\).


%% The fully random experiment extends \(f\) and \(f'\) to larger sets \(S' = (S_1', \dots, S_k')\) and \(S' \cup S_{k+1}'\).
%% We still require that \(f(x, \cdot) = f(y, \cdot)\) for any \(x,y\) in the same partition of \(S'\), and likewise for \(f'\). Further, \(f'\) must still be a subselector of \(f\).
%% Let the sets selected by \(f\) from \(S'\) and \(f'\) from \(S' \cup S_{k+1}'\) in this experiment be \((B_1, \dots, B_k)\) and \((B_1', \dots, B_{k+1}')\).

%% The following lemma describes how domination between the first pair of selections carries through to the second pair, given a slightly refined error-event.

%% \begin{lemma}
%%   Let \(\calE\) be an event such that \((A_1, \dots, A_k) \preceq_\calE (B_1, \dots, B_k)\).
%%   Then \[(A_1', \dots, A_{k+1}') \preceq_{\calE'} (B_1', \dots, B_{k+1}')\]
%%   for \(\calE' = \calE \cap \parentheses{A'_{k+1} \leq B_{k+1}'} \cap \calI\parentheses{\bigcup_{i=1}^k A_i}\).
%% \end{lemma}



%% Let \(f\) be a selector function defined on a set \(S\) and \(f'\) be a subselector of \(f\), defined on a larger set \(Z \supseteq S\).


%% We consider a partition of each universe, \(S = (S_1, \dots, S_k), Z=(Z_1, \dots, Z_k)\)

%% Let \(A\) be a set of selected elements, partitioned into sets \(A = (A_1, \dots, A_k)\) such that, within each \(A_i\), all elements are compared against the same set of bitmasks -- in other words, for \(x, y \in A_i\), we require \(f(x, \cdot) = f(y, \cdot)\), and denote this function by \(f_i\).

%% For each \(i\), let \(f_i'\) be a subselection of \(f\) such that \(A' = (A_1', \dots, A_k')\) is a subselection of \(A\).


%% Let \(B = (B_1, \dots, B_k)\) be a family of sets and \(\calE\) be an event such that \(A \preceq_\calE B\).

%% We will use the following observation to argue that stochastic dominance between one pair of selections will carry over to the next pair, with an added error event.


%% \begin{observation}
%%   Let \(A\) be the set of elements selected by tornado tabulation, and \(B\) be the set of elements selected by the same selectiong function using fully random hashing.
%%   Partition \(A, B\) into families \(\calA=(A_1, \dots, A_k)\) and \(\calB=(B_1, \dots, B_k)\) in such a way that, for each \(i\), all elements of \(A_i \cup B_i\) are chosen based on the same bitmasks.
%%   Assume there exists an event  \(\calE\) such that \(\calA \preceq_\calE \calB\).

%%   For each \(i\), let \(A_i'\) be a subselection of \(A_i\), and let \(B_i'\) be the same subselection of \(B_i\).

%%   Finally, let \(A_{k+1}', B_{k+1}'\) be a selection, by tornado tabulation and full randomness respectively, of keys not considered for the prior selection.

%%   Then
%%   \[(A_1', \dots, A_{k+1}') \preceq_{\calE'} (B_1', \dots, B_{k+1}')\]
%%   for \(\calE' = \calE \cap \parentheses{A_{k+1}' \leq B_{k+1}'} \cap \calI(A_k)\).
%% \end{observation}

\subsection{Selections and segments}
We divide the elements of input set \(S\) into different \emph{segments} based on their weight, defining \(S_i = \set{x_k \in S : p_k \in (2^{-(i+1)},\, 2^{-i}]}\) for each \(i \in \set{0, \dots, \log \size{\calR}}\).
Thus elements of \(S_0\) are \emph{very} likely to be sampled, while those of \(S_{\log \size{\calR}}\) most likely won't.

If an element \(x \in S_i\) is sampled, we can thus infer that \(h(x) < \size{\calR} / 2^i\), and thus the bit-representation of \(h(x)\) is prefixed by at least \(i\) \texttt{0}'s.
On the other hand, if \(x \in S_i\) is \emph{not} sampled then \(h(x) \geq \size{\calR} / 2^{i+1}\) and the bit-representation of the hash value is prefixed by at most \(i\) \texttt{0}'s.

We will perform a total of \(\log \size{\calR}\) selections, with the \(i\)'th selection using the first \(i\) bits as selection bits.
We assign each segment to a \emph{level} \(L_i\), such that segments of \(L_i\) are included from the \(i\)'th selection and up.
The levels are defined as described in \cref{define-levels}.

\begin{algorithm}[H]
  \SetKwData{KwIdx}{index}
  \SetKwData{KwCap}{capacity}
  \(\KwIdx \gets 0\)\;
  \For{\(i = 0\) \KwTo \(\log\size{\calR}\)}{
    \(\KwCap \gets 2^i \cdot \ssigma/6\) \;
    \(L_i \gets \emptyset\)\;
    %% \While{dummy}{text}\;
    \While{\(\size{L_i} + \size{S_{\KwIdx}} \leq \KwCap\)}{
      \(L_i \gets L_i \cup S_{\KwIdx}\)\;
      \(\KwIdx \gets \KwIdx + 1\)\;
    }
  }
  \caption{Defining levels.}\label{define-levels}
\end{algorithm}

The \(i\)'th selection consists of three parts:
\begin{description}
\item [New keys, \(N_i\).]
  Keys from level \(L_i\) are selected into \(N_i\) if all \(i\) select bits are \texttt{0}'s.
\item [Continuing keys, \(R_i\).]
  A key from \(\bigcup_{j<i} L_j\) (the set considered for \(N_{i-1} \cup R_{i-1}\)) is included in \(R_i\) if all \(i\) select bits are \texttt{0}'s.
\item [Final keys, \(F_i\).]
  A key from segment \(S_j\) for \(j < i\) is included in \(F_i\) the first \(j\) select bits are \texttt{0}'s,
\end{description}

We want the following to be true (\jonas{TODO}):
\begin{lemma}
  Let \(k = \log \size{\calR}\).
  The events \(\parentheses{h(x_i) < p_i}_{x_i \in F_k}\) are independent when conditioned on \(F_k\), and \(\Prpcond{h(x_i) < p_i}{x_i \in F_k} = p_i \cdot 2^\ell\) for \(x_i \in S_\ell\).
\end{lemma}

\subsection{Concentration of a weighted sum}
As a step towards concentration bounds on the number of Poisson Samples we extend our concentration bounds to the setting of weighted sums.

Consider a set of \(n\) elements \(\calU = \set{x_1, \dots, x_n}\) with each element having an associated weight \(w_i\) such that \(0 \leq w_1 \leq w_2 \leq \dots \leq w_n\).
Let \(X = \set{ x_i \in \calU : h(x) \leq p}\) for some threshold \(p\).
When \(h\) is tornado tabulation \cref{thm:pretty1,thm:Chernoff-upper} give concentration bounds for \(\size{X}\).
Through the following two lemmas we extend this to a guarantee on \(\sum_{x_i \in X} w_i\) which is concentrated around \(p \cdot \sum_{i \in [n]} w_i\).

We use the notation \(\calU_{\geq t}\) to denote the set \(\set{x_i \in \calU : w_i \geq t}\), and analogously for \(X_{\geq t}\).

\begin{lemma}
  If \(\Delta_1, \dots, \Delta_n\) are values such that \(\size{X_{\geq w_i}} \leq p \cdot \size{\calU_{\geq w_i}} + \sum_{j\geq i} \Delta_j\) for all \(i \in [n]\),
  then
  \[
  \sum_{x_i \in X} w_i \leq \sum_{i \in [n]} w_i (p+\Delta_i) \, .
  \]
\end{lemma}
\begin{proof}
  Let \(w_0 = 0\). Using that \(w_i \geq w_{i-1}\) we have
  \begin{align*}
    \sum_{x_i \in X} w_i
    &= \sum_{i=1}^n (w_i - w_{i-1}) \size{X_{\geq w_i}} \\
    &\leq \sum_{i =1}^n (w_i - w_{i-1}) \cdot \parentheses{p \cdot \size{\calU_{\geq w_i}} + \sum_{j =i}^n \Delta_j} \\
    &\leq p \sum_{i =1}^n (w_i - w_{i-1}) \cdot \size{\calU_{\geq w_i}} + \sum_{i=1}^n (w_i - w_{i-1}) \cdot \sum_{j=i}^n \Delta_j \\
    &= p\sum_{i=1}^n w_i + \sum_{j=1}^n \Delta_j \cdot \sum_{i=1}^j (w_i - w_{i-1}) \\
    &= p\sum_{i=1}^n w_i + \sum_{j=1}^n w_j \Delta_j \, .
  \end{align*}
\end{proof}

